A Predict-Then-Optimize Customer Allocation Framework for Online Fund Recommendation

With the rapid growth of online investment platforms, funds can be distributed to individual customers online. The central issue is to match funds with potential customers under constraints. Most mainstream platforms adopt the recommendation formulation to tackle the problem. However, the traditional recommendation regime has its inherent drawbacks when applying the fund-matching problem with multiple constraints. In this paper, we model the fund matching under the allocation formulation. We design PTOFA, a Predict-Then-Optimize Fund Allocation framework. This data-driven framework consists of two stages, i.e., prediction and optimization, which aim to predict expected revenue based on customer behavior and optimize the impression allocation to achieve the maximum revenue under the necessary constraints, respectively. Extensive experiments on real-world datasets from an industrial online investment platform validate the effectiveness and efficiency of our solution. Additionally, the online A/B tests demonstrate PTOFA's effectiveness in the real-world fund recommendation scenario.

==> section/abstract.tex <==
\begin{abstract}

Online investment platforms are watching growth rapidly, which enables the distribution of mutual funds to individual customers online. The central issue is to match funds with potential customers. In the real world, most mainstream platforms adopt the recommender system to tackle the problem. However, observing several disadvantages introduced by top-\textit{k} recommendation, we conclude that the traditional recommendation fails to meet the demands of both customers and fund managers. In this paper, we model the fund distribution matching as an allocation task. Following the predict-then-optimize manner, we design the Expected Revenue Optimized (ERO) framework. The data-driven framework consists of two stages, prediction and optimization, which aim to predict expected transaction value based on customer behavior and optimize the impression allocation to achieve the maximum revenue under the necessary constraints. Extensive experiments on real-world datasets from an industrial online investment platform validate the effectiveness and efficiency of our solution. Additionally, the online A/B tests also demonstrate the effectiveness of EOCA in the real-world fund recommendation scenario.

%Online investment platforms facilitated by digital payments are watching growth rapidly, which enable the distribution of mutual funds personalized to individual investors via mobile Apps. As the important intermediation of financial products investment, these platforms distribute thousands of mutual funds obtaining impressions under guaranteed delivery (GD) strategy required by fund companies. Driven by the profit from fund purchases of customers, the platform aims to maximize each transaction amount of customers by promoting mutual funds to these investors who will be interested in. Different from the conversions in traditional advertising or e-commerce recommendations, the investment amount in each purchase varies greatly even for the same financial product, which provides a significant challenge for the promotion recommendation of mutual funds. In addition to predicting the click-through rate (CTR) or the conversion rate (CVR) as in traditional recommendations, it is essential for FinTech platforms to estimate the customers' purchase amount for each delivered fund and achieve an effective allocation of impressions based on the predicted results to optimize the total expected transaction value (ETV). In this paper, we propose an ETV-optimized customer allocation framework (EOCA) that aims to maximize the total ETV of recommended funds, under the constraints of GD dealt with fund companies. EOCA consists of two phases: a prediction phase of the customer purchase amount followed by a constrained allocation phase. Specifically, we propose an entire space deep probabilistic model with a novel-designed loss function to predict the purchase amount when a promotional fund is exposed to a customer, which involves not only the conversion rate prediction but also the post-conversion purchase amount estimation. Based on the predicted ETV, we design a heuristic algorithm to solve the large-scale constrained combinatorial optimization problem to suggest which fund each customer should be exposed to in order to maximize the total purchase amount. To the best of our knowledge, it's the first attempt to solve the GD problem for financial product promotions based on customer purchase amount prediction. We conduct extensive experiments on large-scale real-world datasets and online tests based on LiCaiTong, Tencent’s wealth management platform, to demonstrate the effectiveness of our proposed EOCA framework.
\end{abstract}

==> section/methodology_old.tex <==
\section{methodology}
\label{sec:methodology_old}

An effective expected transaction value (ETV) prediction is the essential premise to achieve the optimal or near-optimal transaction value during a delivery period. Figure \ref{fig:workflow} presents an illustrative example of customer allocation for guaranteed delivery in the financial distribution platform. In this instance, two promotional funds are required to be delivered to three users. Fund $f_1$ demands two allocated users for impression, and fund $f_2$ is planned to deliver to one user according to the predetermined contract between the FinTech platform and fund company. Firstly, the framework needs to estimate the $ETV_{i,j}$ for each $u_i$ and $f_j$. Secondly, the framework solves the customer allocation problem where the predicted ETV is used as the constant. This provides a challenging large-scale combinational optimization solution that involves over 10 million users and a variety of funds. As the example shown in Figure \ref{fig:workflow}, one on hand, the conventional top-k recommendation will fail to satisfy the GD constraints since all three users prefer  $f_1$.  On the other hand, the manual allocation strategy can easily lead to a sub-optimal solution: i) if it firstly satisfies the impression requirement of $f_1$, $u_1$ and $u_2$ will be allocated to $f_1$ and thus $u_3$ is allocated to $f_2$ for delivery. The total ETV, in this case, is 510 + 900 + 300 = 1710; ii) if it firstly satisfies $f_2$, $f_2$ will be delivered to $u_2$ and $f_1$ will be delivered to $u_1$ and $u_3$, ETV = 600 + 510 + 500 = 1610. However, the optimal solution shown in Figure \ref{fig:workflow} is allocating $u_2$ and $u_3$ to $f_1$ and $u_1$ to $f_2$, with the maximum ETV 1850. 

\subsection{Entire Space Deep Probabilistic Model}
Accurately estimating the ETV requires the model to address two main tasks: i) predict whether the user will purchase the delivered item, and ii) if the conversion occurs, predict how much money the user is willing to invest. Thus, we formulate the ETV as the product of click \& conversion rate (CTCVR) and the expected revenue after conversion:
\begin{equation}
    ETV = \underbrace{Pr(click) \times Pr(conversion| click) }_{CTCVR} \times \mathbb{E}(R),
    \label{ETV} 
\end{equation}
where R is the revenue bought by the customer. 

We denote $v$ as the result of the following logarithmic transformation applied to the R:
\begin{equation}
    v=\left\{
    \begin{aligned}
        &\log (R + 1)  , &  PA > 0 \\
        &0  , & R = 0
    \end{aligned}
    \right.
\end{equation}
Note that in order to avoid confusion between positive samples with an amount of 1 and those without conversion, we added 1 to the purchase amount of all samples, and the processed revenue label is denoted as $y_v = R + 1$ and thus $v = \log(y_v)$. 

The first task is a typical classification problem, which has been discussed in many previous works. Nevertheless, there are several significant challenges for predicting customer purchase amounts, and we doubt that the existing methods based on MSE loss or ZILN loss can effectively solve this problem in practice. In addition to the zero inflation phenomenon caused by a large number of non-converted samples, the difference in the purchase amount of converted samples is also very large. 
\begin{figure} \centering    
    \subfloat[The distribution of overall positive samples.] {
        \label{fig:a}
        \includegraphics[width=0.46\columnwidth]{figure/distri_overall2}  }     
    \subfloat[Distributions of three users' histroical logarithmic transaction value.] { 
        \label{fig:b}
        \includegraphics[width=0.47\columnwidth]{figure/distri_4}}    
    \caption{ Distribution of logarithmic transaction value. }     
    \label{distribution}     
\end{figure}
Figure \ref{distribution} shows the logarithmic transaction value of converted samples of the real-world financial transactions data. It implies that the converted users' log transaction values follow a normal distribution. Especially besides the overall distribution of overall converted samples, we present examples of the historical purchase amount distribution of three different users in Figure \ref{fig:b}. Users 1 and user 3 have similar profiles and behaviour patterns. Yet both of them are quite different from user 2. Meanwhile, the logarithmic transaction value distributions of users 1 and 3 are similar, while the distribution of user 2 is significantly different from theirs. Therefore, inspired by the ZILN loss, we assume that the observed log purchase amount $v_i$ of each positive sample $i$ for a financial product is sampled from an implicit normal distribution. The parameters of the distribution, i.e. the mean $\mu$ and the standard deviation $\sigma$, are determined by the sample's features.

\subsubsection{Entire Sample Space Modeling} Different from the conventional e-commerce scenario, due to investment risks, users need a longer time to consider before making final decisions. Some users have developed a strong willingness to purchase a fund even though they have not converted yet. Moreover, for guaranteed delivery, models need to infer both pCTCVR and post-conversion purchase amounts on the entire sample space, including new-coming users. This requires the models to be trained with supervision for both tasks on the entire sample space. Otherwise, the performance of models in practical applications will suffer from sample selection bias in the actual industrial environment.

In order to tackle this problem, we provide a novel perspective of sample space division that unifies the classification and regression tasks for financial recommendation scenarios, as shown in Figure \ref{samplespace}. For the convenience of understanding, we introduce a hidden variable $C$, $C = 1$ means that the user has the willingness to convert for the delivered mutual fund, and $C = 0$ indicates that the user has no intention to purchase. Note that if the conversion is observed, it means that C = 1, while users might have the intention to convert even for observed negative samples. We assume that the probability of the event $C=1$ is approximately equal to pCTCVR and
\begin{equation}
\begin{aligned}
    P(v| C = 1, \mu,\sigma) \approx P(v| y = 1, \mu, \sigma) 
    = \frac{1}{\sqrt{2\pi}\sigma y_v }\exp({-\frac{(v- \mu)^2}{2\sigma ^2}})
\end{aligned}
\end{equation}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/entiresamplespace.pdf}
    \caption{The entire sample space division.}
    \label{samplespace}
\end{figure}


\begin{figure*}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/EOCA_3.pdf}
    \caption{The ETV-optimized customer allocation (EOCA) framework. For the ETV prediction phase, EOCA uses the ESDPM architecture as shown in the left part, which is trained with our novel-designed entire space multi-task joint (ESJ) loss. With the predicted ETV as the constraint, EOCA solves the large-scale customer allocation problem with a heuristic algorithm under the GD constraints.}
    \label{model}
\end{figure*}


For a given data set with each point described as  $(\vec{x_u}, \vec{x_f}, y, v ) $, where $\vec{x_u}$ is features of user $u$ and $ \vec{x_f}$ is features of fund $f$, we summarize the sample space as:

\begin{itemize}
    \item User $u$ purchases the delivered fund $f$ and thus $C=1$ and $y = 1$. The observed transaction amount $v \textgreater0$. (Sample subspace $\mathcal{R}_1$)
    \item User $u$ has no intention to purchase ($C = 0$) and thus $y = 0$ and $v = 0$. (Sample subspace $\mathcal{R}_2$)
    \item User $u$ has the intention to purchase ($C=1$) while has not purchased yet and the observed transaction amount $v = 0$. (Sample subspace $\mathcal{R}_3$)
\end{itemize}
Samples in the subspace $\mathcal{R}_1$ are observed positive samples, and samples in subspaces  $\mathcal{R}_2$ and  $\mathcal{R}_3$ are all observed negative samples. We utilize a multi-task probabilistic model to fit the data set. The first main task is to model the probability of a purchase event occurring,  and the second main task is to learn the parameters $\mu$ and standard deviation $\sigma$ of each sample's implicit normal distribution, thereby estimating the probability of the event occurring which the sample's observed logarithmic transaction value is $v$ under the condition that C = 1. 

In this way, the probability of an observed positive sample with a user-fund pair $i$ that involves user $u$ and fund $f$ can be formulated as:
\begin{equation}
	\begin{aligned}
		& P(C = 1,y = 1, v = v | \vec{x_{u}}, \vec{x_{f}}) \\ 
		& = P(y = 1, v = v | \vec{x_{u}}, \vec{x_{f}}) \\
		&= P(y  = 1 | \vec{x_{u}}, \vec{x_{f}})  \times P(v| \vec{x_{u}}, \vec{x_{f}} , y  = 1) \\
		& = pCTCVR \times \frac{1}{\sqrt{2\pi}\sigma_i y_{vi} }\exp({-\frac{(v_i - \mu_i)^2}{2\sigma_i ^2}})
		\label{positive} 
	\end{aligned}
\end{equation}
The probability of observed negative sample $P(y  = 0, v = 0 | x_{u}, x_{f})$ can be formulated as:
\begin{equation}
	\begin{aligned}
		& P(y = 0, v = 0 | \vec{x_{u}}, \vec{x_{f}}) \\ 
		& = P(C = 0, y = 0, v = 0 | \vec{x_{u}}, \vec{x_{f}}) \\
		& +   P(C = 1, y = 0, v = 0 | \vec{x_{u}}, \vec{x_{f}}) \\
		& \approx (1 - pCTCVR) + pCTCVR \times \frac{1}{\sqrt{2\pi}\sigma_i y_{vi}}\exp({-\frac{ \mu_i^2}{2\sigma_i ^2}}) 		
		\label{negative} 
	\end{aligned}
\end{equation}
Therefore, the likelihood of ESDPM with trainable parameters set $\Theta$ and data set $\mathcal{D}$ can be written as:

\begin{equation}
	\begin{aligned}
		\mathcal{P}(\mathcal{D};\Theta)   & =  \prod_{ i \in \mathcal{R}_1} P( C = 1, y = 1, v = v| \vec{x_{u_i}},\vec{x_{f_i}}  )   \\
		\times & \prod_{ j \in \mathcal{R}_2 \cup \mathcal{R}_3}  ( P( C = 0, v = 0| \vec{x_{u_j}},\vec{x_{f_j}} )\\
		&\qquad \quad	+ P( C = 1, v = 0| \vec{x_{u_j}},\vec{x_{f_j}} ) )
		\label{likehood} 
	\end{aligned}
\end{equation}


According to Equation \ref{positive} - \ref{likehood}, we can finally derive the following form of entire space multi-task joint (ESJ) loss function from the negative log-likelihood loss function: 

\begin{equation}
	\begin{aligned}
		\mathcal{L} & = -\frac{1}{M}(\sum_{ i,y_i = 1 } \log ( P(y = 1, v = v_i | \vec{x_{u_i}}, \vec{x_{f_i}}) ) \\
		& \quad  \quad +\sum_{ j, y_j = 0 } \log(P(y = 0, v = 0 | \vec{x_{u_j}}, \vec{x_{f_j}}) )	\\
		& = -\frac{1}{M}(\sum_{ i,y_i = 1 }( \log p +  \log \frac{1}{\sqrt{2\pi} \sigma_i y_{v_i}} +({-\frac{(v_i - \mu_i)^2}{2\sigma_i ^2}})) \\
		&\quad  \quad  + \sum_{j, y_j = 0 }(  \log  (1- p   +  p \times \frac{1}{\sqrt{2\pi}\sigma_j y_{vj}}\exp({-\frac{\mu_j ^2}{2\sigma_j ^2}}))))
		\label{loss function} 
	\end{aligned}
\end{equation}
where we denote pCTCVR as $p$. Through the proposed loss function ESJ, the model has a joint probability modelling of the classification task and regression task on the entire sample space. With the predicted $pCTCVR_{uf}$, parameters of the log-normal distribution $\mu_{uf}$ and $\sigma_{uf}$ the predicted expected transaction value when fund $f$ is delivered to user $u$ can be written as:
\begin{equation}
	\begin{aligned}
		{ETV} = pCTCVR_{uf} \times \exp(\mu_{uf} + \sigma_{uf}^2/2)
		\label{final etv} 
	\end{aligned}
\end{equation}

\subsubsection{Model Architecture}The aforementioned problems require our proposed ESDPM model to accurately estimate the customers' investment intention and the amount they plan to invest. How much money a user is planning to use for investment is not only related to the user's investment intention and investment habits but also directly related to the user's available capital. 

To tackle these challenges, on one hand, we use the widely used self-attention mechanism\cite{vaswani2017attention} to capture the users' investment habits based on their historical behaviour data, i.e. click funds, purchase, sell and add to favourites, in the sequential manner. On the other hand, we construct a consumption graph $G = (\mathcal{V}, \mathcal{E})$ to better estimate users' post-conversion purchase amount. The consumption graph is a bipartite graph, while the nodes in the graph consist of user nodes $\mathcal{V}_U$ and merchant nodes $\mathcal{V}_M$. There is an edge between a user $u$ and a merchant $m$ if $u$ has paid to $m$.  Graph neural networks (GNNs) are proven to be effective for extracting information from graph data and have been widely used \cite{kipf2016semi,hamilton2017inductive,huang2019text,hong2020attention,guo2020deep}. The user's payment behaviour to different merchants contains valuable information and implies the user's available capital in a way. In addition, applying the two-layer GNN model to the user-merchant-user graph can help the model capture the information of a target user through the attributes of users who have similar consumption behaviour patterns. For an illustrative example, the occupation of a new user is unknown, and the user often consumes in a canteen during workdays. The occupation information of other users who consume in the canteen simultaneously can help the model infer the user’s occupation. In this way, consumption graph data help ESDPM better understand users so as to better meet their needs of wealth management. Without loss of generality, we utilize graph attention layer \cite{DBLP:journals/corr/abs-1710-10903} to help ESDPM focus on the important information of consumption graph. 

Figure \ref{model} presents the architecture of ESDPM.   It firstly generates the user embedding $\mathbf{e_u}$ and fund embedding $\mathbf{e_f}$ via concatenating the feature embeddings of the user and fund respectively. The user behaviour embedding $\mathbf{e_b}$ and consumption embedding $\mathbf{e_c}$ are then generated by the self-attention layer and graph attention layer. Finally, we concatenate them into a vector as input:
\begin{equation}
	\begin{aligned}
		\mathbf{e} = [\mathbf{e_u} \parallel \mathbf{e_f} \parallel	\mathbf{e_b} \parallel	\mathbf{ e_c}]	
		\label{input embedding} 
	\end{aligned}
\end{equation}
After that, ESDPM feeds the generated input vector to the subsequent multi-task learning network. Here we adapt the structure of MMoE \cite{ma2018modeling} to capture the relationships between tasks. The post-click conversion rate is learned as a hidden variable as ESMM\cite{ma2018entire}. We can obtain the ETV according to the output of ESDPM and the equation (\ref{final etv}). 

\subsubsection{Discussion}
For plain multi-task learning models, including binary classification tasks and continuous values regression tasks, cross-entropy loss and MSE loss remain dominant presence\cite{liu2018joint,gutelman2020efficient}, and the final loss is obtained by simply adding the losses of the above-mentioned two tasks. This form of multi-task loss function does not consider classification and regression tasks in a unified sample probability space but essentially models these two tasks separately. Besides, it ignores the variance differences of the samples' regression label distributions and is sensitive to outliers during the training process. Therefore, the performance of MTL models with such a loss function might be limited. 

ESJ loss divides the unconverted samples into two situations: i) no intention to convert ($\mathcal{R}_2$), ii) willing to convert but the investment amount is 0  ($\mathcal{R}_3$). Through such a reasonable distinction of samples,  the classification task and regression task are unified in the entire sample space and make the model perform supervised regression training for the observed negative samples. In addition, ESJ formulates the probability of each sample based on the assumption that the transaction value labels are heteroscedastic in terms of different samples. The ZILN loss function only considers $\mathcal{R}_2$ for the observed negative samples, which implies that the purchase amount of the samples that have the intention to convert must be greater than 0. It can be proved that under the assumption that the regression label follows normal distributions, ZILN loss denoted by $\mathcal{L}_{ZILN}$ is a special case of the loss function we proposed:
\begin{equation}
	\begin{gathered}
		\label{prove}
		P(\mathcal{R}_3)  = p \times \frac{1}{\sqrt{2\pi}\sigma_j y_{vj}}\exp({-\frac{\mu_j ^2}{2\sigma_j ^2}}) \equiv 0 \\
		\Downarrow \\
		\mathcal{L} =  -\frac{1}{M}[\sum_{i ,y_i = 1 }( \log p + \log \frac{1}{\sqrt{2\pi }\sigma_i y_v{vi}}+  ({-\frac{(v_i - \mu_i)^2}{2\sigma_i ^2}})) \\
		\qquad \qquad + \sum_{j , y_j = 0 }(  \log  (1- p   +   P(j \in \mathcal{R}_3)))] \\	
		=  -\frac{1}{M}[\sum_{ i}{ (y_i \log p + (1-y_i)\log (1-p) )}  + \sum_{ j,y_j  = 1} \mathcal{L}_{R}(j) ] \\
=\mathcal{L}_{ZILN}	
	\end{gathered}
\end{equation}
where $\mathcal{L}_{R}(j) = -\frac{(v_j - \mu_j)^2}{2\sigma_j ^2} + \log \frac{1}{\sqrt{2\pi}\sigma_j y_{vj}}$ is the supervised regression loss for observed positive samples. The formulation of ZILN loss shows that it uses the cross-entropy loss for classification tasks training on the entire sample space, while the regression loss is only used for positive samples. Since ZILN loss has no regression supervision for the observed negative samples and needs to meet the implicit condition of $P(j \in \mathcal{R}_3) = 0$, it is easy for the model to erroneously overestimate the $\mu_i$ of the logarithmic purchase amount distribution for samples in the inference space.

\subsection{Large Scale Customer Allocation Solution}

With the estimated ETV as the constraint,  the remaining task of the EOCA framework is to solve the allocation problem described in Section 2. Although there are some commercial tools for solving constrained integer programming problems, according to previous work \cite{ji2021large} and the attempts we have made, these commercial solvers cannot solve large-scale allocation problems in a reasonable time. Moreover, the strict risk constraint and strict constraint that the number of allocated users for each fund must exactly equal to the demand require a special design allocation algorithm for large-scale guaranteed delivery in FinTech platforms. 
\begin{algorithm}
    \caption{Heuristic Optimization Algorithm}\label{algorithm}
    \KwIn{ETV,  \\
        T = \{$t_i$|$\forall i, {u_i\in U} $\}; \\  R =\{$r_j$ |${f_j\in F}$\}; \\D = \{$d_j$ |${f_j\in F}$\}
    }
    \KwOut{$\mathbf{X}$}
    
    $ETV_{i,j} \leftarrow 0 , \forall i\forall j r_j > t_i$\;
    \For{j = 1 to $|F|$}{$\alpha_j \leftarrow  \frac{ \sum_{i} ETV_{i,j}}{d_j} $}
    \For{i = 1 to $|U|$}{
        Sort $\{f_j| \forall j\leq|F|\}$ in descending order based on $ETV_{i,j}$\;
        Select the top-3 highest scored funds $a,b,c$\;
        $h_i \leftarrow  \frac{\alpha_a + \alpha_b}{2} \times (2\times ETV_{i,a} - ETV_{i,b} - ETV_{i,c}   );$
    }
    Sort $\{u_i| \forall i\leq|U|\}$ in descending order based on $\{h_i\}$\;
    \While{$i \leq |U| $}{
        Select the highest scored fund $a$ of $u_i$, $X_{ia} \leftarrow 1$ \;
        $U \leftarrow U  \backslash  u_i$ \; 
        $d_a \leftarrow d_a - 1$ \;
        \If{$d_a$ = 0}{$\forall i, ETV_{i,a} \leftarrow 0 $\;
            Execute from line 2 to line 10;
        }
    }
\end{algorithm}

\subsubsection{Description of our proposed allocation algorithm}
We summarize the proposed heuristic optimization algorithm (HA) in Algorithm \ref{algorithm}. In Line 1, we set $ETV_{i,j} $ to 0 if the risk tolerance level of user $u_i$ is lower than risk level of fund $f_j$. We introduce the factor $\alpha_j$ to estimate the satisfaction speed of the fund $f_j$ during the allocation process. If $\alpha_j$ of the fund j is larger than that of other funds, it implies that the fund $f_j$ may reach the allocated user number limit sooner, and other remaining users cannot be allocated to $f_j$ at that time. Based on $\alpha$ and ETV, the algorithm calculates the heuristic score $h$ for each user in Line 5 to Line 9. Firstly, for the user $u_i$, sort all funds in descending order of ETV to get the top 3 funds $ a,b,c$. Secondly, respectively calculate the score difference between $ETV_{i,a}$ and $ETV_{i,b}$ as well as the score difference between $ETV_{i,a}$ and $ETV_{i,c}$, get $\Delta_1 $ and $\Delta_2$, and finally get $ h_{i} = \frac{\alpha_a + \alpha_b}{2}(\Delta_1 + \Delta_2)$. $h_{i}$ measures the decrease of objective function that may result if the user $i$ is not allocated to the current highest-scored fund in time. In Line 10, the algorithm sorts all users in descending order according to the calculated $h$. The part from Line 11 to Line 19 executes the allocation process, the user with the highest $h_i$ is allocated to the fund $a$ with the highest ETV refer to $u_i$ and remove $u$ from the unallocated user set $U$. If the $d_a$ is satisfied, the algorithm sets the $ETV_{k,a}$ to 0 for all remaining users and recalculates $\alpha$ and $h$. Repeat the loop until all users are allocated. 

\subsubsection{Discussion}
The higher the heuristic score $h_i$ for a user $u_i$ is, the more prominent the user’s preference for a certain promotional fund. If the allocation strategy fails to allocate $u_i$ to the fund that obtains the highest ETV regard to $u_i$, it probably leads to a more obvious loss for the objective value. In other words, the HA strategy tends to conduct delayed allocation for the users who have similar preferences for all $k$ promotional funds. Besides, the algorithm ensures that exact $d_j$ users are allocated to each promotional fund $j$, and users will not be allocated to the fund with a higher risk level than the user's risk tolerance. In the problem of GD in financial scenarios, the number of users that are allocated to each product must be exactly equal to demand due to the consideration of the balance between overall risk control and profit. 
Although recent research used solvers based on Lagrangian methods to achieve near-optimal solutions for the constrained optimization problem in practical applications\cite{zhang2020request,li2020spending}, these existing approaches can hardly ensure no constraints will be violated after allocation.


